Beyond Cats and Dogs: Semi-supervised Classification of fuzzy labels with overclustering

A long-standing issue with deep learning is the need for large and consistently labeled datasets. Although the current research in semi-supervised learning can decrease the required amount of annotated data by a factor of 10 or even more, this line of research still uses distinct classes like cats and dogs. However, in the real-world we often encounter problems where different experts have different opinions, thus producing fuzzy labels. We propose a novel framework for handling semi-supervised classifications of such fuzzy labels. Our framework is based on the idea of overclustering to detect substructures in these fuzzy labels. We propose a novel loss to improve the overclustering capability of our framework and show on the common image classification dataset STL-10 that it is faster and has better overclustering performance than previous work. On a real-world plankton dataset, we illustrate the benefit of overclustering for fuzzy labels and show that we beat previous state-of-the-art semisupervised methods. Moreover, we acquire 5 to 10% more consistent predictions of substructures.

==> Paperv2-flattened- beforeClean_arXiv/images.tex <==
\graphicspath{{images/}}

\newcommand{\picSmall}[3]{
	\begin{figure}[tb] 
		\centering
		\includegraphics[width=#3\linewidth]{#1}
		\caption{#2}
		\label{fig:#1}
	\end{figure}
}

\newcommand{\picTwo}[4]{
	\begin{figure*}[tb]
		\centering
		\begin{subfigure}[c]{0.49\textwidth}
			\centering		
			\includegraphics[width=0.9\textwidth]{#1-0}
			\subcaption{#2}	
			\label{fig:#1-0}	
		\end{subfigure}
		\begin{subfigure}[c]{0.49\textwidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-1}
			\subcaption{#3}
			\label{fig:#1-1}	
		\end{subfigure}
		\caption{#4}
		\label{fig:#1}
	\end{figure*}
}

\newcommand{\picTwoHor}[4]{
	\begin{figure}[tb]
		\centering
		\begin{subfigure}[c]{0.49\textwidth}
			\centering		
			\includegraphics[width=0.9\textwidth]{#1-0}
			\subcaption{#2}	
			\label{fig:#1-0}	
		\end{subfigure}
		\begin{subfigure}[c]{0.49\textwidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-1}
			\subcaption{#3}
			\label{fig:#1-1}	
		\end{subfigure}
		\caption{#4}
		\label{fig:#1}
	\end{figure}
}

\newcommand{\picThree}[5]{
	\begin{figure*}[tb]
		\centering
		\begin{subfigure}[c]{0.32\textwidth}
			\centering		
			\includegraphics[width=0.9\textwidth]{#1-0}
			\subcaption{#2}		
		\end{subfigure}
		\begin{subfigure}[c]{0.32\textwidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-1}
			\subcaption{#3}		
		\end{subfigure}
		\begin{subfigure}[c]{0.32\textwidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-2}
			\subcaption{#4}		
		\end{subfigure}
	
		\caption{#5}
		\label{fig:#1}
	\end{figure*}
}

\newcommand{\picFour}[3]{
	\begin{figure*}[htb]
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#1-0}
		\end{subfigure}
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#1-1}
		\end{subfigure}
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#1-2}
		\end{subfigure}
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#1-3}
		\end{subfigure}	
		
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#2-0}
		\end{subfigure}
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#2-1}
		\end{subfigure}
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#2-2}
		\end{subfigure}
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#2-3}
		\end{subfigure}	
		\caption{#3}
		\label{fig:#1}
	\end{figure*}
}

\newcommand{\picTwelve}[2]{
	\begin{figure*}[htb]
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-00}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-01}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-02}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-03}
		\end{subfigure}			
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-04}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-05}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-06}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-07}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-08}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-09}
		\end{subfigure}
		
		
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-10}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-11}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-12}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-13}
		\end{subfigure}			
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-14}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-15}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-16}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-17}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-18}
		\end{subfigure}
		\begin{subfigure}[c]{0.09\textwidth}		
			\includegraphics[width=\textwidth]{#1-19}
		\end{subfigure}
	
	
		\caption{#2}
		\label{fig:#1}
		
	\end{figure*}
}

==> Paperv2-flattened- beforeClean_arXiv/tables.tex <==
\newcommand\doubletable[2]{
\begin{table}
	\centering
	
	\begin{minipage}{.48\linewidth}
		#1
	\end{minipage}%
	\hfill
	\begin{minipage}{.48\linewidth}
		#2		
	\end{minipage}%
\end{table}
}

\newcommand{\tblOne}{
	\doubletable{\tblComparisonSTL}{\tblComparisonPlankton}
}
\newcommand{\tblTwo}{
	\doubletable{\tblConsistency}{\tblPretextTask}
}
\newcommand{\tblThree}{
	\doubletable{\tblAblationStl}{\tblAblationPlankton}
}

\newcommand{\tblPretextTask}{
\begin{table}
	
	
	
	
	\centering
	\resizebox{0.85\linewidth}{!}{%
		
		\begin{tabular}{l c c c c }
			\toprule
			& & \multicolumn{2}{c}{Accuracy} &    \\ 
			\cmidrule(r){3-4}
			Method  & r & Overcluster & Normal & Runtime \\ 
			\midrule				
			IIC \cite{iic} & - &   63.1 & & -- \\
			
			\midrule 
			
			IIC* & - & 59.31 & & 114 h \\
			FOC  & 0 &  57.28 & 48.10 & \textbf{10 h}\\
			FOC  & 0.5 &  59.24 & \textbf{52.96} & 13 h\\
			FOC & 1& \textbf{64.44} & 50.92  & 89 h \\
			
			\midrule
			
			FOC$^\dagger$ & 1 & 72.06 & 69.83 & 81 h \\
			
			\bottomrule
		\end{tabular}
		
	}
	
	\caption{Pretext task on STL-10 -- 
		$r$ indicates the restriction of unlabeled data.
		The runtime is the training time in hours on the same hardware.
		The best results are marked bold.
		A horizontal line indicates different comparisons. 				
		Legend: * Original authors code used. 
		$^\dagger$ Uses supervised augmentations and can be seen as upper bound estimation.
	}
	\label{tbl:unsupervised-pretext-stl10}
	\vspace{-4mm}
\end{table}
}

\newcommand{\tblAblationStl}{
	\begin{table}
	
	
	\centering
	
	\resizebox{\linewidth}{!}{%
		\begin{tabular}{l c c c c c c}
			\toprule
			& & & & & \multicolumn{2}{c}{Accuracy}     \\ 
			\cmidrule(r){6-7}
			Method & Pre & MI & \ceinv &  Weight &    Overcluster & Normal \\
			\midrule
			FOC  &  & X& & -- &   75.71 & 76.46 \\	
			IIC* \cite{iic} &  X  & & & -- &   & 85.76 \\				
			FOC  &  X & X &  & -- & 74.19 & 86.05 \\	
			FOC &  X & X& X & -- &  82.69& 86.49 \\		
			FOC  &  X & X & X & C &  \textbf{85.54} & \textbf{86.98}\\
			FOC  & X & X&X & I & 83.70 & 85.25 \\
			
			\bottomrule
		\end{tabular}
	}
	
	\caption{Ablation study on STL-10 -- 
		The second to fourth column indicates if a pretext task as pretraining, the mutual information loss and our novel loss \ceinv was used respectively.
		The fifth column indicates the weights used for initialization.
		C stands for Cifar-20 and I for ImageNet.
		If no weight initilization is given, sobel filtered images are used as input.
		Legend: * Original authors code.
		The best results are marked bold.
	}
	\label{tbl:AblationStl}
	
\end{table}
}

\newcommand{\tblComparisonSTL}{
\begin{table}
	
		
		\centering
		
		\resizebox{\linewidth}{!}{%
			\begin{tabular}{l l  c c}
				\toprule
				& &  \multicolumn{2}{c}{Accuracy}     \\ 
				\cmidrule(r){3-4}
				Method & Network &  Overcluster & Normal  \\ 
				\midrule		
				ADC \cite{adc}  & ResNet &  &  77.0 \cite{iic} \\ 	
				SCAN$^\star$ \cite{scan} & ResNet18 & & 80.9 \\			
				IIC* \cite{iic} & ResNet34 &  & 85.76 \\	
				CMC$^\dagger$  \cite{cmc} & AlexNet &  & 86.88 \\ 	
				FOC (Ours) & ResNet34 &  85.54 & 86.98 \\
				IIC$^\dagger$ \cite{iic} & ResNet34 &  & 88.8 \\
				MixMatch$^\ddagger$ \cite{mixmatch}  & Wide ResNet28 &  & 89.82 \\
				MixMatch \cite{mixmatch} & Wide ResNet28 &  & 94.41 \\
				FixMatch$^\ddagger$ \cite{fixmatch} & Wide ResNet28 &  & 94.83 \\
				
				\bottomrule
			\end{tabular}
		}
		
		
			\caption{Comparison to state-of-the-art on STl-10  -- The results are reported in the original paper or the link is given behind the value.  Legend: * Original authors code without MLP for fine-tuning.
			$^\dagger$ A MLP used for fine-tuning.
			$^\ddagger$ Used only 1000 labels instead of 5000.
			$^\star$ Unsupervised method.
		}
		\label{tbl:comparisonSTL}
\end{table}
}	
		
		
\newcommand{\tblAblationPlankton}{
\begin{table}
	
	
		\centering
		
		\resizebox{\linewidth}{!}{%
			\begin{tabular}{l c c c c c c c c}
				\toprule
				& & & & &  \multicolumn{2}{c}{Accuracy} &   \multicolumn{2}{c}{F1-Score}     \\ 				
				\cmidrule(r){6-7}  \cmidrule(r){8-9} 
				Method & Pre & MI & \ceinv &  Weight &    Overcluster & Normal &  Overcluster & Normal  \\ 
				\midrule
				
				IIC  & X &  &  & -- &  -- & 74.25 & -- & \textbf{66.63} \\
				IIC$^\dagger$ & X &  &  & -- &  -- &  78.71 &  -- & \textbf{69.92}  \\		
				
				\midrule
				
				FOC & & &  & C & 51.17 & 59.31 & 31.45 & 38.70 \\
				FOC & & X & & C & 58.24 & \textbf{79.28} & 32.27 & 60.66 \\
				FOC & & X & X & C  & 78.66  & 76.68 & 71.70 & 64.23 \\
				
				\midrule
				FOC & X & &  & C & 55.64 & 73.94 & 27.64 & 59.84 \\
				FOC& X & X& & C & 80.63 & 75.12 & 70.37 & 56.67 \\
				FOC & X & X & X & C  & \textbf{82.25} & 77.64 & 70.57 & 58.12 \\
				
				\midrule
				
				FOC & & & & I & 55.21 & 74.69 & 29.57 & 54.92 \\		
				FOC & & X & & I & 80.43 & 78.42 & \textbf{72.34} & 64.80 \\
				FOC &  & X& X & I & \textbf{81.48} & 78.81 & \textbf{73.52} & 64.85 \\
				
				\midrule
				FOC & X & &  & I & 59.87 & 74.73 & 39.54 & 55.54 \\
				FOC & X & X & & I & 80.63 & \textbf{80.48} & 70.66 &  66.47 \\
				FOC & X & X & X & I &   \textbf{83.11}  & \textbf{79.00} & \textbf{77.60}  & \textbf{67.23}  \\
				
				\bottomrule
			\end{tabular}
		}
	    
	    \caption{Ablation study on plankton dataset --
		The second to fourth column indicate if a pretext task as pretraining, the mutual information loss and our novel loss \ceinv was used respectively.
		The fifth column indicates the weights used for initialization.
		C stands for Cifar-20 and I for ImageNet.
		If no weight initilization is given, sobel filtered images are used as input.
		The best three results are marked bold.
		Legend: 
			$^\dagger$ A MLP used for fine-tuning.
		}	
			\label{tbl:AblationPlankton}
    		
\end{table}
}

\newcommand{\tblComparisonPlankton}{
\begin{table}
		\centering
		
	
		
		
		\resizebox{\linewidth}{!}{%
			\begin{tabular}{l  c c c c}
				\toprule
				Method	& \# Classes &  F1-Score & Accuracy\\
				
				\midrule
				
				
				SCAN$^\star$ \cite{scan} & 10 & 38.34 & 62.54  \\	
				SCAN$^\star$ \cite{scan} & 60 & 38.15 & 62.16   \\		
				IIC \cite{iic} & 10 & 66.63 &  74.25   \\
				IIC$^\dagger$ \cite{iic} & 10 & 69.92 &  78.71   \\				
				Mean-Teacher \cite{mean-teacher}  & 10 & 74.51 & 81.06   \\
				Pi \cite{temporal-ensembling} & 10 & 74.03 & 81.09  \\
				Pseudo-label \cite{pseudolabel} & 10  & 75.14 & 81.12 \\
				FixMatch \cite{fixmatch} & 10 & 75.97 & \textbf{83.14} \\		
				FOC (Ours) &  10 & 67.23  &  79.00  \\
				FOC (Ours) &  60 & \textbf{77.60} &  \textbf{83.11} &   \\
				
				
				\bottomrule
			\end{tabular}	
		}
		
			\caption{Comparison to state-of-the-art on plankton dataset -- 
			The results were calculated on the unlabeled data which include the fuzzy labels.
			The number of classes indicates the usage of overclustering (60 classes).	
			The accuracy is provided for comparison but can be misleading due to class imbalance.
			All results within a one percent margin of the best result are marked bold. 
			Legend:
			$^\dagger$ A MLP used for fine-tuning.
			 $^\star$ Unsupervised method.
		}
		\label{tbl:comparisonPlankton}
		
		\vspace{-4mm}
		
\end{table}
}			
		
\newcommand{\tblConsistency}{	
\begin{table}
	
		
		
		\centering
		
		\resizebox{\linewidth}{!}{%
		\begin{tabular}{l c c c c }
			\toprule
	
			& \multicolumn{2}{c}{all data}  & 	\multicolumn{2}{c}{ignore class no-fit} \\ 
			
			\cmidrule(r){2-3} \cmidrule(r){4-5}
			Method  & overall & per cluster & overall & per cluster \\
			\midrule				
			
			
			FixMatch \cite{fixmatch} &  82.56 & 78.78 $\pm$ 28.22 & 77.11 & 69.61 $\pm$ 29.41 \\
			FOC (Ours) &\textbf{87.80} & \textbf{79.66 $\pm$ 18.88} & \textbf{86.31} & \textbf{86.41 $\pm$ 13.68}\\
			
			\bottomrule
		\end{tabular}
		}
		
		\caption{Consistency comparison on plankton dataset --
		    The consistency is rated by experts over the complete data and a subset without the mixed class no-fit.
		    An image is consistent with the cluster if it is rated by an expert as similar with the majority of the cluster.
		    We provide the percentage of consist data overall and as average with standard deviation per cluster.
		    Further information about the calculations are provided in \autoref{subsec:consistency}.
		    }
		 \label{tbl:consistency} 
		 
		 \vspace{-4mm}
		   
\end{table}

	
		    
}


\newcommand{\tblAblation}{	
\begin{table}
	\centering
	
	\begin{minipage}{\linewidth}
		\resizebox{\linewidth}{!}{%
		\begin{tabular}{l c c c c c c}
			\toprule
			& & & & & \multicolumn{2}{c}{Accuracy}     \\ 
			\cmidrule(r){6-7}
			Method & Pre & MI & \ceinv &  Weight &    Overcluster & Normal \\
			\midrule
			FOC  &  & X& & -- &   75.71 & 76.46 \\	
			IIC* \cite{iic} &  X  & & & -- &   & 85.76 \\				
			FOC  &  X & X &  & -- & 74.19 & 86.05 \\	
			FOC &  X & X& X & -- &  82.69& 86.49 \\		
			FOC  &  X & X & X & C &  \textbf{85.54} & \textbf{86.98}\\
			FOC  & X & X&X & I & 83.70 & 85.25 \\
			
			\bottomrule
		\end{tabular}
	}
	\subcaption{STL-10}
	
	\end{minipage}%
	\hfill
	\begin{minipage}{\linewidth}
		\resizebox{\linewidth}{!}{%
			\begin{tabular}{l c c c c c c c c}
				\toprule
				& & & & &  \multicolumn{2}{c}{Accuracy} &   \multicolumn{2}{c}{F1-Score}     \\ 				
				\cmidrule(r){6-7}  \cmidrule(r){8-9} 
				Method & Pre & MI & \ceinv &  Weight &    Overcluster & Normal &  Overcluster & Normal  \\ 
				\midrule
				
				IIC \cite{iic}  & X &  &  & -- &  -- & 74.25 & -- & \textbf{66.63} \\
				IIC$^\dagger$ \cite{iic} & X &  &  & -- &  -- &  78.71 &  -- & \textbf{69.92}  \\		
				
				\midrule
				
				FOC & & &  & C & 51.17 & 59.31 & 31.45 & 38.70 \\
				FOC & & X & & C & 58.24 & \textbf{79.28} & 32.27 & 60.66 \\
				FOC & & X & X & C  & 78.66  & 76.68 & 71.70 & 64.23 \\
				
				\midrule
				FOC & X & &  & C & 55.64 & 73.94 & 27.64 & 59.84 \\
				FOC& X & X& & C & 80.63 & 75.12 & 70.37 & 56.67 \\
				FOC & X & X & X & C  & \textbf{82.25} & 77.64 & 70.57 & 58.12 \\
				
				\midrule
				
				FOC & & & & I & 55.21 & 74.69 & 29.57 & 54.92 \\		
				FOC & & X & & I & 80.43 & 78.42 & \textbf{72.34} & 64.80 \\
				FOC &  & X& X & I & \textbf{81.48} & 78.81 & \textbf{73.52} & 64.85 \\
				
				\midrule
				FOC & X & &  & I & 59.87 & 74.73 & 39.54 & 55.54 \\
				FOC & X & X & & I & 80.63 & \textbf{80.48} & 70.66 &  66.47 \\
				FOC & X & X & X & I &   \textbf{83.11}  & \textbf{79.00} & \textbf{77.60}  & \textbf{67.23}  \\
				
				\bottomrule
			\end{tabular}
		}
		
		\subcaption{plankton dataset}
	    
	   	
	\end{minipage}%
	
	 \caption{Ablation study on STL-10 and plankton dataset --
		The second to fourth column indicate if a pretext task as pretraining, the mutual information loss and our novel loss \ceinv was used respectively.
		The fifth column indicates the weights used for initialization.
		C stands for Cifar-20 and I for ImageNet.
		If no weight initilization is given, sobel filtered images are used as input.
		The best results are marked bold for STL-10 and the best three for plankton dataset.
		Legend: 
		    * Original authors code 
			$^\dagger$ A MLP used for fine-tuning.
		}	
			\label{tbl:Ablation}	
			
	\vspace{-4mm}
\end{table}
		    
}
